Bear the Query in Mind: Visual Grounding with Query-conditioned Convolution

Visual grounding is a task that aims to locate a target object according to a natural language expression. As a multi-modal task, feature interaction between textual and visual inputs is vital. However, previous solutions mainly handle each modality independently before fusing them together, which does not take full advantage of relevant textual information while extracting visual features. To better leverage the textual-visual relationship in visual grounding, we propose a Query-conditioned Convolution Module (QCM) that extracts query-aware visual features by incorporating query information into the generation of convolutional kernels. With our proposed QCM, the downstream fusion module receives visual features that are more discriminative and focused on the desired object described in the expression, leading to more accurate predictions. Extensive experiments on three popular visual grounding datasets demonstrate that our method achieves state-of-the-art performance. In addition, the query-aware visual features are informative enough to achieve comparable performance to the latest methods when directly used for prediction without further multi-modal fusion.

==> figures/refcoco_example.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\linewidth]{images/refcoco383.png}
  \caption{Query and image target example. \hw{this paper will probably be read by the community that is familiar with grounding, so this figure does not really tell anything important. Please consider removing it. }}
  \label{fig:refcoco-example}
\end{figure}
% \begin{wrapfigure}{r}{0.5\linewidth}
%     \centering
%     \includegraphics[width=5cm]{}
%     \caption{Query and image target example.}
%     \label{fig:refcoco-example}
% \end{wrapfigure}

==> figures/same-img-atten-diff.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{images/same-img-atten-diff.png}
  \caption{Attention weights constructed from different queries of the same image in TransVG+DyConv. The left two queries ``woman in red dress" and ``lady red" have similar attention weight distributions, and the right three queries ``man in striped shirt on bike", ``striped shirt" and ``stripped shirt" have similar attention weight distributions.}
  \label{fig:same-img-atten-diff}
\end{figure}

==> figures/vis-regtoken.tex <==
\begin{figure}[H]
    \centering
    
    \subfloat[TransVG]{
    	\label{subfig:sfig1}
    	\includegraphics[width=0.95\linewidth]{images/vltransformer-transvg.png} }
    	
    \subfloat[VGQC w/ fusion]{
    	\label{subfig:sfig2}
    	\includegraphics[width=1\linewidth]{images/vltransformer-dconv.png} }
    	
    \subfloat[VGQC w/o fusion]{
    	\label{subfig:sfig3}
    	\includegraphics[width=1\linewidth]{images/regtoken-nofusion.png} }
    	
    \caption{We show the [REG] token's attention to visual tokens at different layers. In \ref{subfig:sfig1} and \ref{subfig:sfig2}, we visualize the [REG] in the fusion module. In \ref{subfig:sfig3}, we visualize the [REG] token in the VGQC w/o fusion. \textcolor{green}{Green} boxes are the ground truth labels and \textcolor{red}{red} boxes are the predicted labels. The last column are the queries.}
    \label{fig:vis-regtoken}

\end{figure}

==> figures/vis-resnet.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{images/vis-resnet.2.jpg}
  \caption{Comparison of feature maps from ResNet across different models and text queries.}
  \label{fig:vis-resnet-feature-map}
\end{figure}

==> sections/backup-5-analysis.tex <==
\section{Analysis}


\subsection{Ablation Study}
The result in Table~\ref{tab:attention-ablation} proves that performance improvement is resulted from incorporating text into convolution kernel generation. Simple convolution kernel generated without text information cannot improve the accuracy.
\input{tables/attention-ablation}

The results in Table~\ref{tab:layer-ablation} and Table~\ref{tab:num-kernel-ablation} provide the optimal hyperparameter setting of replacing 3 layers of ResNet and using 5 candidate kernels in each query-conditioned convolution block. 

\input{tables/layer-ablation}
\input{tables/num-kernel-ablation}

\subsection{Analysis of Query-conditioned Convolution Kernel}
By visualizing the attention weights and the aggregated kernel of each query-conditioned convolution block, we show that the attention weights and the aggregated kernels effectively embed textual semantic meanings. In particular, the aggregated kernels behave in a similar manner as text embeddings such that aggregated kernels contracted from similar text queries are closer to each other in the aggregated kernel’s semantic space. 

\input{figures/blue-red-atten}

\input{figures/same-img-atten-diff}

There are 20 query-conditioned convolution blocks in our CNN backbone and each block has an attention weight vector with length $K=5$. We find that in the first 15 attention weights, the attention distributions are generally even, and the activation of a particular attention weight in the first half layers represents special text information. For example, Figure~\ref{fig:blue-red-atten} shows the heat maps of the 20 attention weighs derived from different queries in VGQC w/ fusion model. When the queries contain “blue”, the last attention weight in the query-conditioned convolution block {\#6} is activated with value greater than 0.7, which is the attention weight in the first bottleneck block of the second layer of ResNet. When the queries contain “red”, the last attention weight in the query-conditioned convolution block {\#10} is activated with value greater than 0.7, which is the attention weight of the downsampling convolution block of the third layer of ResNet. By lowering the activation threshold from 0.7 to 0.5, most queries that activate the last attention weight of the query-conditioned convolution block {\#6} contains “blue” and “yellow”, and “jeans” can also activate it as it has the semantic information of “blue” in its text embedding. Most queries that activate the last attention weight of the query-conditioned convolution block {\#10} contains “red”, “pink” and “purple”. Furthermore, Figure~\ref{fig:same-img-atten-diff} shows the attention weights of the same image with different queries in VGQC w/ fusion model. The queries “women in red dress” and “lady red” have similar attention patterns while the rest of the queries with “man” and “striped shirts” have similar attention distributions. 

Similar patterns appear in VGQC w/o fusion model. The last attention weight in the query-conditioned convolution block {\#6} can still detect "blue" and "yellow", but the last attention weight in the query-conditioned convolution block {\#10} is not activated by "red" anymore. However, we don't find any attention weight activated by "left" or "right" in  VGQC w/ fusion, but the first attention weight in the query-conditioned convolution block {\#8} in  VGQC w/o fusion model can response to "right" in queries. By removing the fusion module, the candidate kernels and the aggregated kernels are forced to learn more information from text. Therefore, it is proved that the attention weight in each the query-conditioned convolution block effectively encodes textual information. 

We also find that the attention weight distribution is usually unbalanced in the last 4 attention weights, which means the attention is more focused on one of the five candidate kernels in the last several the query-conditioned convolution blocks. This may be because as the CNN gets deeper, candidate kernels are more expressive and can represent more abstract high-level features, so a single candidate kernel with high attention weight in the last several blocks can successfully extract enough features from the previous feature map. It also implies that the candidate kernels are diverse enough such that each candidate kernel extracts different aspects of features with different significance. 

\input{tables/dynamic-kernel-reference}

\input{tables/dynamic-kernel-eachother}

In addition to attention weights, the aggregated kernels also contain significant text information as shown in Table~\ref{tab:dynamic-kernel-reference} and Table~\ref{tab:dynamic-kernel-eachother}. We use the same image in Figure~\ref{fig:same-img-atten-diff} and pass different queries into our models. Different attention weights and the five candidate kernels are taken from the query-conditioned convolution block {\#10}. A reference kernel is built by assigning equal weights to every candidate kernel, i.e. the average of the five candidate kernels. Then, we calculate the cosine distance of the aggregated kernels of different queries from the reference kernel in Table~\ref{tab:dynamic-kernel-reference}. “woman in red dress” and “lady red” have their last attention weight activated, so they are the furthest away from the reference kernel and the remaining aggregated kernels are closer. 

In addition, the cosine distances between the aggregated kernels of different queries are shown in Table~\ref{tab:dynamic-kernel-eachother}. “woman in red dress” and “lady red” are very close to each other, and they have the same distance away from “woman”. “woman in red dress” have very different semantic meanings from “man in striped shirt on bike” and “striped shirt”, so its aggregated kernel is far away from the other two while the other two aggregated kernels are closer. This proves that the aggregated convolution kernels embed meaningful textual information in its aggregated kernel semantic space in a similar way as text embeddings in the textual semantic space. This distance relationship holds regardless of the particular information represented by attention weights and candidate kernels.

\subsection{Feature Map Difference}
The key strength of our model is the use of query-conditioned convolution. This allows the ResNet backbone to produce query-aware feature maps given different text queries for a single image. To understand the extent of this phenomenon, we examine the output feature map $z \in \mathcal{R}^{{C}\times{H}\times{W}}$ from the last layer of ResNet, where $C=2048$, $H=20$, and $W=20$. We compute $\bar{z} \in \mathcal{R}^{\times{H}\times{W}}$ which is the average of $z$ across $C$, and plot it as a heat map.

\input{figures/vis-resnet}

Figure~\ref{fig:vis-resnet-feature-map} visualizes the comparison of $\bar{z}$ across different models and text queries. Given a fixed image input, we observe that the feature map from the original ResNet in TransVG is query oblivious, i.e., it does not change across different text queries. In contrast, the outputs from our approaches are query dependent. It is worth noting that in the case of  VGQC w/o fusion, the locations of the image targets (the purple shirt and gray shirt) actually correspond to the locations with the highest values (colored in white) in the feature maps. Since the feature maps of ResNet have been shown to implicitly encode absolute positional information ~\cite{islam2020position}, we believe this indicates that the aggregated convolution kernels are capturing visual information relevant to the text query.

% We also try overlaying the feature maps from our on model on top of the input image, since the feature maps of ResNet have been shown to implicitly encode absolute positional information ~\cite{islam2020position}. To our surprise, important areas of the image targets (here the pink shirt and blue shirt) actually correspond to high output values in the heat maps. We believe this is an indicator that the dynamic convolution kernels are capturing information relevant to the text query.

\subsection{[REG] Token Attention at Different Layers}
To see the relationship between visual attention and predicted bounding box, we visualize the attention of the [REG] token to visual tokens in the fusion module in all six layers. Figure~\ref{fig:vis-regtoken} compares the attention between the original TransVG and our proposed VGQC w/ fusion. It can be observed that with the help of query-conditioned convolution in the visual branch, attentions in the fusion module are more dense. We notice that in the first layer, the [REG] token in the original TransVG captures the global context, while our proposed method has attention on referred object already. In the middle layers, both models attend to the object(s) mentioned in the query. In the last layer, the attention spreads out to formulate the region of the bounding box.

\input{figures/vis-regtoken}

==> sections/method.tex <==
% \section{Experimental Setup}
\input{figures/framework}
\xl{figure2 can (a)(b) can be drawn in one figure.}
\section{Methodology}
As shown in Figure~\ref{fig:framework}, our model can be boiled down to four parts: a textual encoder, a text-guided visual encoder, an optional visual-linguistic feature fusion module and a prediction head.

\paragraph{Textual Encoder.}
Textual encoder aims to extract query Following previous works \cite{}, we utilize 
\paragraph{Text-guided visual encoder.}
\paragraph{Fusion module.}
\paragraph{Prediction head.}

\subsection{Visual Encoder with Query-conditioned Convolution}
The visual encoder in VGQC is composed of a CNN backbone with query-conditioned convolution blocks and transformer encoders. The query-conditioned convolution blocks compose convolution kernels according to the input text query, so that such convolution kernels extract target-relevant features from the previous feature map. As shown in Figure~\ref{fig:aggregated-kernel_block}\xl{Figure~\ref{}, Table~\ref{}, add $\sim$}, in each block, there are $K$ candidate convolution kernels $\{\boldsymbol{\tilde{w}}_1, \boldsymbol{\tilde{w}}_2,..., \boldsymbol{\tilde{w}}_K\}$ of the same size. 
% Each candidate kernel extracts a different set of features from the input feature map.
Each candidate kernel represents a particular set of features to be extracted from the feature map, and text queries with different semantic meanings may require different combinations of these sets of features. 
Therefore, the candidate kernels are aggregated according to an attention weight $\boldsymbol{\alpha}=[\alpha_1, ..., \alpha_K]$ computed from the query sentence representation $\boldsymbol{f}_{query} \in \mathcal{R}^{L_q}$ with length denoted as $L_q$. The attention weight $\boldsymbol{\alpha}$ is calculated by projecting $\boldsymbol{f}_{query}$ into a $K$-dim vector using two linear layers and a softmax layer:
\begin{equation}
   \boldsymbol{\alpha} = \text{softmax}(g(\boldsymbol{f}_{query}))
\end{equation}
\begin{equation}
    \boldsymbol{\tilde{W}} = \sum^{K}_{i = 1}\alpha_i\boldsymbol{\tilde{w}}_i
\end{equation}
where $g$ is a linear transformation unique for each query-conditioned convolution block. 



With this approach, both the attention weight $\boldsymbol{\alpha}$ and the aggregated kernel $\boldsymbol{\tilde{W}}$ contain textual information. The aggregated kernel $\boldsymbol{\tilde{W}}$ is then used to replace regular kernels in the CNN backbone. Such convolution block can be applied to replace an arbitrary number of kernels at arbitrary layers in the CNN backbone.

In our visual encoder, we choose ResNet ~\cite{he2015deep} as the CNN backbone and replace the first convolution kernel of each bottleneck block in one or more ResNet layers with query-conditioned convolution blocks. With input image of size $\mathcal{R}^{3\times{H}\times{W}}$, the output feature map from ResNet is $\boldsymbol{z} \in \mathcal{R}^{2048\times{\frac{H}{32}}\times{\frac{W}{32}}}$. Next, the output channel dimension of 2048 is reduced to 256 by convolution, transforming $\boldsymbol{z}$ into $N_v$ primary visual tokens $\boldsymbol{z}_v \in \mathcal{R}^{256\times{N_v}}$ where $N_v = \frac{H}{32}\times \frac{W}{32}$. Then, $\boldsymbol{z}_v$ is passed into a stack of 6-layer transformer encoders in a similar way as DETR encoder ~\cite{carion2020endtoend}. A fixed sine positional embedding is added to $\boldsymbol{z}_v$ before each transformer encoder. There are 8 heads in the transformer encoder's multi-head self-attention layer. The transformer encoder's hidden dimension is 256, and the FFN dimension is 2048. Finally, the output of the query-conditioned visual encoder is a set of query-aware visual tokens $f_v \in \mathcal{R}^{L_v\times{N_v}}$, where the length of each token $L_v$ is 256.
\xl{figure should appear before section 3.1}
\input{figures/aggregated-kernel_block}

\subsection{Query-conditioned Framework for Visual Grounding}
With the query-conditioned visual encoder, we propose a visual grounding framework VGQC with an optional fusion module. First, the textual encoder extracts textual features from the query and produces a sentence representation $\boldsymbol{f}_{query}$ along with a group of textual tokens $\boldsymbol{f}_q$. 
% There is no structure limitation for the textual encoder. 
The query-conditioned visual encoder takes in both $\boldsymbol{f}_{query}$ and the input image to produce a group of query-aware visual tokens $\boldsymbol{f}_v$. The following fusion module takes in the textual tokens $\boldsymbol{f}_q$ and the query-aware visual tokens $\boldsymbol{f}_v$ to perform multimodal feature fusion. Finally, a multimodal feature representation from the fusion module is fed into the prediction head and gets directly regressed to the coordinates of the target bounding box. The VGQC framework is flexible in terms of the choice of the text encoder, CNN backbone in the visual encoder, and the fusion module. The entire model is trained in an end-to-end manner.

In our experiments, we use BERT ~\cite{devlin2019bert} as the textual encoder and take the output [CLS] embedding as the query representation $\boldsymbol{f}_{query} \in \mathcal{R}^{L_q}$. The textual tokens are $\boldsymbol{f}_q \in \mathcal{R}^{L_q\times{N_q}}$ where $N_q$ is the number of textual tokens and the length of each token $L_q$ is 768. Our proposed query-conditioned visual encoder takes in the image and $\boldsymbol{f}_{query}$ to generate a group of query-aware visual tokens $\boldsymbol{f}_v \in \mathcal{R}^{L_v\times{N_v}}$. For the fusion module, we adopt the visual-linguistic fusion module from TransVG ~\cite{deng2021transvg} which passes the textual tokens $\boldsymbol{f}_q$ and visual tokens $\boldsymbol{f}_v$ through two separate linear projectors and a stack of 6-layer transformer encoders with a learnable regression token [REG] $\in \mathcal{R}^{256}$ appended at the front. The output [REG] embedding is fed into the prediction head which is a 2-layer fully connected neural network with 256 hidden units and ReLU activation followed by an output linear layer. The prediction head directly regresses the input to the 4 coordinates of the target bounding box.

We also propose a VGQC framework that removes the fusion module. 
%Since the query-aware visual tokens $\boldsymbol{f}_v$ are informative enough to eliminate the need for the fusion module. 
We use BERT as the textual encoder and feed $\boldsymbol{f}_{query}$ into the query-conditioned visual encoder. In the visual encoder, a learnable regression token [REG] $\in \mathcal{R}^{256}$ is appended in front of the primary visual tokens $\boldsymbol{z}_v$ before fed into the transformer encoders. The output [REG] embedding is a representation of all the query-aware visual tokens and gets passed into the prediction head to generate the bounding box coordinates.  

\subsection{Training Objective}
The training objective is the GIoU loss plus a smooth L1 loss. Let $A(S)$ denote the area covered by a bounding box $S$, and let $S_i$ and $\hat{S}_i$ be the ground-truth and predicted bounding boxes for sample $d_i$, respectively. Intersection-over-Union (IoU) ratio is calculated as:
\begin{equation}
    IoU_i = \frac{A(S_i \cap \hat{S}_i )}{A(S_i \cup \hat{S}_i )}
\end{equation}
In Generalized IoU ~\cite{rezatofighi2019generalized}, let $S_c$ denote the smallest convex object enclosing $S_i$ and $\hat{S}_i$, and GIoU is calculated as:
\begin{equation}
    GIoU_i = IoU_i - \frac{A(S_c) \setminus A(S_i \cup \hat{S}_i)}{A(S_c)}
\end{equation}
where $\setminus$ means the area of $A(S_c)$ excluding $A(S_i \cup \hat{S}_i )$.
GIoU loss is $L_{GIoU}=1-GIoU$. The smooth L1 loss is calculated between the ground truth coordinated and the predicted coordinates normalized by the size of image. The training objective is to minimize the overall loss $L$:
\begin{equation}
    L = L_{GIoU} + L_{smooth_{l1}}
\end{equation}

==> tables/acc_main_old.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lrrrrrrrrr}
\hline
                & \multicolumn{3}{c}{RefCOCO} & \multicolumn{3}{c}{RefCOCO+} & \multicolumn{3}{c}{RefCOCOg} \\
                & val      & testA   & testB   & val      & testA    & testB   & val-g     & val-u  & test-u  \\ \hline
TransVG (reported)  & 80.32    & 82.67   & 78.12   & 63.50    & 68.15    & 55.63   & 66.56     & 67.66   & 67.44    \\
TransVG (reproduced)  & 80.18    & 82.53   & 75.25   & 65.47    & 70.09    & 57.20   & 66.23     & todo   & todo    \\
VGQC w/ fusion  & 82.47    & 85.02   & 77.98   & running  & running  & running & 68.7   & 67.95   & 67.89    \\
VGQC w/o fusion & 80.01    & 83.02   & 73.94   & 66.37    & 73.11    & 56.50   & 62.32     & todo   & todo    \\ \hline
\end{tabular}

\caption{Performance of our main models}
\label{tab:acc_main}
\end{table*}



==> tables/attention-ablation.tex <==
\begin{table}
\centering
\begin{tabular}{lrrr}
\toprule
Models                 & val   & testA & testB \\
\midrule
TransVG                   & 80.18 & 82.53 & 75.25 \\
VGQC w/ fusion - method 1 & 80.81 & 82.44 & 76.33 \\
VGQC w/ fusion - method 2 & 80.66 & 82.42 & 75.39 \\
VGQC w/ fusion            & \textbf{82.47} & \textbf{85.02} & \textbf{77.98} \\
\bottomrule
\end{tabular}
\caption{Ablation study on generating QCM's attention weight with different methods on RefCOCO dataset. 1) method 1: attention weight $\boldsymbol{\alpha}$ is a randomly initialized, learnable K-dimensional vector parameter. 2) method 2: the attention weight $\boldsymbol{\alpha}$ is derived from the previous feature map. 3) The attention weight is derived from the text query in original VGQC.}

\label{tab:attention-ablation}
\end{table}

==> tables/candidate-kernel-ablation.tex <==
\begin{table}[]
\centering
\begin{tabular}{lrrrrrr}
\toprule
      & All & \#1 & \#2 & \#3 & \#4 & \#5  \\ \hline
val   & 69.17 & 54.80    &  43.54   & 58.73    & 57.55    & 55.76     \\
testA & 73.52 & 57.28    &  30.73   & 58.66    & 58.69    & 58.87     \\
testB & 58.97 & 49.96    &  55.83   & 54.48    & 57.55    & 49.94      \\ \hline
\end{tabular}


% \begin{tabular}{lrrrrrr}
% \toprule
%      & Mean & -\#1 & -\#2 & -\#3 & -\#4 & -\#5  \\ \hline
% val  & 64.71 & 64.87 & 67.17 & 68.70 & 69.08 & 64.99  \\
% testA  & 67.88 & 66.59 & 72.20 & 73.03 & 73.31 & 66.53  \\
% testB & 57.54 & 58.57 & 55.09 & 58.73 & 59.14 & 59.30 \\ \hline
% \end{tabular}
\caption{Overall accuracy (\%) on RefCOCO+ when VGQC w/ fusion uses only one candidate kernel or masks one candidate kernel out in the final QCM block. For example, \#1 means using only the first candidate kernel, and -\#2 means masking the second candidate kernel out. ``Mean" means using a fixed evenly-distributed attention. Their performances are worse than the normal VGQC w/ fusion model (column ``All"). % \chonghan{Is the second table necessary or can be removed?}
}

% \caption{Overall accuracy (\%) on RefCOCO+ when VGQC w/ fusion uses only one candidate kernel or masks one candidate kernel out in the final QCM block. For example, \#1 means using only the first candidate kernel, and -\#2 means masking the second candidate kernel out. ``Mean" means using a fixed evenly-distributed attention. Their performances are worse than the normal VGQC w/ fusion model (column ``All"). \chonghan{Is the second table necessary or can be removed?}}

\label{tab:candidate-kernel-ablation}
\end{table}

==> tables/datasets.tex <==
\begin{table}
\centering
\begin{tabular}{lrrlr} % https://www.tablesgenerator.com/
\toprule
Dataset  & images & queries & split & queries per set \\
\midrule
RefCOCO  & 19,994  & 142,210 & train & 120,624 \\
 & & & val &10,834 \\
 & & & testA & 5,657 \\
 & & & testB & 5,095     \\
RefCOCO+ & 19,992  & 141,564 & train & 120,191 \\
 & & & val & 10,758 \\
 & & & testA & 5,726 \\
 & & & testB &  4,889 \\
RefCOCOg & 25,799  &  95,010  & train-g & 85,474 \\
 & & & val-g &  9,536 \\
  & & & train-u & 80,512  \\
  & & & val-u & 4,896  \\
  & & & test-u & 9,602  \\
\bottomrule
\end{tabular}
\caption{Dataset statistics. RefCOCO and RefCOCO+ are split into train, val, testA and testB sets where testA contains queries only about people whereas
testB contains queries about non-people objects. For RefCOCOg, '-g' means RefCOCOg-google which splits data into train and val set, and '-u' means RefCOCOg-umd which splits data into train, val and test set.}
\label{tab:datasets}
\end{table}

==> tables/dynamic-kernel-eachother-full.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{llrr}
\toprule
Query 1 & Query 2 & VGQC w/ fusion & VGQC w/o fusion \\
\midrule
woman in red dress & woman & 0.3251 & 0.4037 \\
lady red & woman & 0.3345 & 0.5081 \\
woman in red dress & lady red & 0.0001 & 0.0106\\
woman in red dress & man in striped shirt on bike & 0.6117 & 0.3894 \\
woman in red dress & stripped shirt & 0.5794 & 0.2779\\
man in striped shirt on bike & stripped shirt & 0.0112 & 0.0286 \\
stripped shirt & striped shirt & 0.0052 & 0.0143 \\
man in striped shirt on bike & striped shirt & 0.0033 & 0.0025 \\
\bottomrule
\end{tabular}

\caption{The cosine distance of the aggregated kernels in the query-conditioned convolution block {\#10} from each other using the same image with different queries. Similar queries are closer to each other while queries with different semantic meanings are far away from each other.}
\label{tab:dynamic-kernel-eachother-full}
\end{table*}

==> tables/dynamic-kernel-eachother.tex <==
\begin{table}
\centering
\begin{tabular}{llrr}
\toprule
Query1 & Query2 & VGQC(a) & VGQC(b) \\
\midrule
woman in red dress & woman & 0.3251 & 0.4037 \\
lady red & woman & 0.3345 & 0.5081 \\
woman in red dress & lady red & 0.0001 & 0.0106\\
%man in striped shirt on bike & woman in red dress & 0.6117 & 0.3894 \\
%woman in red dress & stripped shirt & 0.5794 & 0.2779\\
woman in red dress & striped shirt & 0.5794 & 0.2779\\
%man in striped shirt on bike & stripped shirt & 0.0112 & 0.0286 \\
%stripped shirt & striped shirt & 0.0052 & 0.0143 \\
\makecell[l]{man in striped shirt \\on bike} & striped shirt & 0.0033 & 0.0025 \\
\bottomrule
\end{tabular}

\caption{The cosine distance of the aggregated kernels from each other in QCM block {\#10} using the same image with different queries. VGQC(a) has a fusion module while VGQC(b) does not use fusion, and they are trained on RefCOCO. %The distances show that aggregated kernels of similar queries are closer to each other, while aggregated kernels of queries with different semantic meanings are far away from each other.
}
\label{tab:dynamic-kernel-eachother}
\end{table}

==> tables/dynamic-kernel-reference-full.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|rl|rl}
\toprule
\multirow{2}{*}{Queries}    & \multicolumn{2}{c}{VGQC w/ fusion} & \multicolumn{2}{c}{VGQC w/o fusion} \\
          & Distance    & Attention weights $(\times 10^{-2})$\    & Distance     & Attention weights $(\times 10^{-2})$   \\
\midrule
woman in red dress & 0.4123 & [ 8.25  8.02  3.00  5.51 75.23] 
& 0.1803 & [42.58 27.95  4.85 17.56  7.04]\\
lady red & 0.4236 & [ 7.77  7.29  2.67  5.38 76.90] 
& 0.2276 & [49.95 23.58  4.52 15.45  6.48]\\
woman & 0.0175 & [14.57 17.50 19.63 23.14 25.16] 
& 0.4638 & [ 5.79 82.70  1.02  7.23  3.24]\\
man in striped shirt on bike & 0.1904 & [47.95 10.32  8.40 19.80 13.53] & 0.4568 & [ 7.44 81.54  1.10  6.81  3.09]\\
stripped shirt & 0.1751 & [44.02  6.75  7.10 24.06 18.07] 
& 0.3321 & [11.77 62.63  1.96 19.94  3.68]\\
striped shirt & 0.2066 & [48.79  6.74  7.46 20.93 16.07] 
& 0.4230 & [ 8.70 75.98  1.15 11.62  2.52] \\
\bottomrule
\end{tabular}
\caption{The cosine distance from the aggregated kernels to the reference aggregated kernel in the query-conditioned convolution block {\#10} using the same image with different queries. The reference aggregated kernel is the unweighted average of the five candidate kernels. Aggregated kernels with and without activated attention are at different distances from the reference kernel.}
\label{tab:dynamic-kernel-reference-full}
\end{table*}

==> tables/dynamic-kernel-reference.tex <==
\begin{table}
\centering
\begin{tabular}{lrr}
\toprule
%\multirow{2}{*}{Queries}    & \multicolumn{2}{c}{VGQC w/ fusion} & \multicolumn{2}{c}{VGQC w/o fusion} \\
%          & Distance    & Attention weights $(\times 10^{-2})$\    & Distance     & Attention weights $(\times 10^{-2})$   \\
Query & VGQC(a) & VGQC(b) \\
\midrule
woman in red dress & 0.4123 %& [ 8.25  8.02  3.00  5.51 75.23] 
& 0.1803 \\%& [42.58 27.95  4.85 17.56  7.04]\\
lady red & 0.4236 %& [ 7.77  7.29  2.67  5.38 76.90] 
& 0.2276 \\%& [49.95 23.58  4.52 15.45  6.48]\\
woman & 0.0175 %& [14.57 17.50 19.63 23.14 25.16] 
& 0.4638 \\%& [ 5.79 82.70  1.02  7.23  3.24]\\
man in striped shirt on bike & 0.1904 %& [47.95 10.32  8.40 19.80 13.53] 
& 0.4568 \\%& [ 7.44 81.54  1.10  6.81  3.09]\\
%stripped shirt & 0.1751 %& [44.02  6.75  7.10 24.06 18.07] 
%& 0.3321 \\%& [11.77 62.63  1.96 19.94  3.68]\\
striped shirt & 0.2066 %& [48.79  6.74  7.46 20.93 16.07] 
& 0.4230 \\%& [ 8.70 75.98  1.15 11.62  2.52] \\
\bottomrule
\end{tabular}
\caption{The cosine distance from the aggregated kernels to the reference kernel in QCM block {\#10} using the same image with different queries. The reference kernel is the unweighted sum of the five candidate kernels in block {\#10}. VGQC(a) has a fusion module while VGQC(b) does not use fusion, and they are trained on RefCOCO. %It can be observed that the aggregated kernels of queries with similar semantic meanings are at the same distance from the reference kernel. Such pattern holds for both VGQC with and without fusion.
}
\label{tab:dynamic-kernel-reference}
\end{table}

==> tables/layer-ablation.tex <==
\begin{table}
\centering
\begin{tabular}{lrrr}
\toprule
Structure                 & val   & testA & testB \\
\midrule
TransVG                   & \textbf{80.18} & 82.53 & \textbf{75.25} \\
VGQC-layer 2\&3\&4  & 80.01 & \textbf{83.02} & 73.94 \\
VGQC-layer 3\&4  & 79.11 & 81.70 & 72.23 \\
VGQC-layer 4  & 78.93 & 82.37 & 73.08 \\
\bottomrule
\end{tabular}
% \caption{Ablation study of different number of query-conditioned convolution blocks by replacing different CNN layers in the backbone ResNet model. The results are from VGQC w/o fusion on RefCOCO dataset. We observe a performance drop when replacing fewer layers with query-conditioned convolution in ResNet.}
\caption{Ablation study on the number of QCM blocks used in the visual encoder. We apply QCM blocks to the selected layers of the backbone ResNet of VGQC w/o fusion and compare the performances on RefCOCO dataset.}
\label{tab:layer-ablation}
\end{table}

==> tables/num-fusion-layer-ablation.tex <==
\begin{table}
\centering
\begin{tabular}{lrrr}
\toprule
Model & val & testA & testB \\
\midrule
TransVG-6-layers        & 80.18 & 82.53 & 75.25 \\
VGQC w/ fusion-6-layers  & 82.47 & \textbf{85.02} & 77.98 \\
VGQC w/ fusion-4-layers  & \textbf{82.67} & 84.54 & \textbf{78.26} \\
VGQC w/ fusion-2-layers  & 81.61 & 84.68 & 76.57 \\
VGQC w/o fusion         & 80.01 & 83.02 & 73.94 \\
\bottomrule
\end{tabular}
\caption{Ablation study on the number of layers used in the fusion transformer on RefCOCO dataset.}
\label{tab:num-fusion-layer-ablation}
\end{table}

==> tables/num-kernel-ablation.tex <==
\begin{table}
\centering
\begin{tabular}{rrrr}
\toprule
K & val & testA & testB \\
\midrule
3 & 79.24 & \textbf{83.04} & 73.69 \\
5 & \textbf{80.01} & 83.02 & \textbf{73.94} \\
8 & 79.05 & 81.96 & 73.23 \\
\bottomrule
\end{tabular}
\caption{Ablation study on different number of candidate kernels (K) in QCM block. The performances of VGQC w/o fusion on RefCOCO dataset are shown.}
\label{tab:num-kernel-ablation}
\end{table}

==> tables/runtime.tex <==
\begin{table}
\centering
\begin{tabular}{lrr}
\toprule
  & Runtime (ms) \\
\midrule
TransVG  & 16.27      \\
VGQC w/ fusion  & 37.46      \\
VGQC w/o fusion  & \textbf{14.81}      \\
\bottomrule
\end{tabular}
\caption{Runtime}
\label{tab:runtime}
\end{table}

==> tables/table_example.tex <==
\begin{table}
\centering
\begin{tabular}{lll}
\hline
Scenario  & $\delta$ & Runtime \\
\hline
Paris       & 0.1s  & 13.65ms     \\
Paris       & 0.2s  & 0.01ms      \\
New York    & 0.1s  & 92.50ms     \\
Singapore   & 0.1s  & 33.33ms     \\
Singapore   & 0.2s  & 23.01ms     \\
\hline
\end{tabular}
\caption{Latex default table}
\label{tab:plain}
\end{table}

% suggest to use booktabs
\begin{table}
\centering
\begin{tabular}{lrr}
\toprule
Scenario  & $\delta$ (s) & Runtime (ms) \\
\midrule
Paris       & 0.1  & 13.65      \\
            & 0.2  & 0.01       \\
New York    & 0.1  & 92.50      \\
Singapore   & 0.1  & 33.33      \\
            & 0.2  & 23.01      \\
\bottomrule
\end{tabular}
\caption{Booktabs table}
\label{tab:booktabs}
\end{table}
